Adversarially Robust Decision Transformer

Decision Transformer (DT), as one of the representative Reinforcement Learning via Supervised Learning (RvS) methods, has achieved strong performance in offline learning tasks by leveraging the powerful Transformer architecture for sequential decision-making. However, in adversarial environments, these methods can be non-robust, since the return is dependent on the strategies of both the decision-maker and adversary. Training a probabilistic model conditioned on observed return to predict action can fail to generalize, as the trajectories that achieve a return in the dataset might have done so due to a suboptimal behavior adversary. To address this, we propose a worst-case-aware RvS algorithm, the Adversarially Robust Decision Transformer (ARDT), which learns and conditions the policy on in-sample minimax returns-to-go. ARDT aligns the target return with the worst-case return learned through minimax expectile regression, thereby enhancing robustness against powerful test-time adversaries. In experiments conducted on sequential games with full data coverage, ARDT can generate a maximin (Nash Equilibrium) strategy, the solution with the largest adversarial robustness. In large-scale sequential games and continuous adversarial RL environments with partial data coverage, ARDT demonstrates significantly superior robustness to powerful test-time adversaries and attains higher worst-case returns compared to contemporary DT methods.

==> 3_theory.tex <==

\subsection{Connection to Nash Q Learning}
In this section, we investigate the connection of minimax expectile regression in the trajectory relabeling of Adversarial Robust Decision Transformer (ARDT) to Nash Q Learning ~\citep{hu2003nash}. We first introduce Nash Q learning, and then show that the return-to-gos learning procedure of ARDT is actually Nash Q learning, which has a convergence guarantee.

Nash Q Learning is designed for solving general-sum stochastic games, but it can be smoothly modified to solve zero-sum Stackelberg Games (with adaptive adversary) in our setting. A stage game is constructed by single step of both protagonist and adversary's action, rewarded by Q values $Q_t$ at current iteration $t$. The Q value function updates of player $i$ in Nash Q Learning is as
\begin{align}
    Q^i_{t+1}(s, a^0, \cdots, a^n) = (1 - \eta_t) Q^i_t(s, a^1, \cdots, a^n) + \eta_t(r_t + \beta \text{Nash}Q^i_t(s')),
\end{align}
for some learning rate $\eta_t$, where $\text{Nash}Q_t(s')=\pi^1(s') \cdots \pi^n(s') \cdot Q^i_t(s')$, and the joint Nash Equilibrium (NE)  of the stage game is denoted by $(\pi^1(s'), \cdots , \pi^n(s'))$ with the payoff functions $Q_t^1(s'), \cdots , Q^n_t(s')$ for $n$ players. In our setting of two-player zero-sum Stackelberg game, the updates of states-action value function of player $i$ becomes
\begin{align}
    Q_{t+1}(s, a, \bar{a}) = (1 - \eta_t) Q_t(s, a, \bar{a}) + \eta_t(r_t + \pi(s', a) \cdot \bar{\pi}(s', a, \bar{a}) \cdot Q^i_t(s')),
    \label{eq_nq}
\end{align}
where the NE of the stage game is 
\begin{align}
    \pi(s') = \arg \max_{\pi' \in \Pi} Q_t(s', a, \bar{a}), \label{eq_nq_max} \\
    \text{s.t.}\ \bar{\pi}(s', a) = \arg \min_{\bar{\pi}' \in \bar{\Pi}} Q_t(s', a, \bar{a}'), \label{eq_nq_min}
\end{align}
where $a \sim \pi'(s'), \bar{a} \sim \bar{\pi}(s', a)$.

Empirically, in ARDT, we parameterize the Q value function by $\omega$ and $\nu$, and update parameters which can also be written in the form of temporal difference in equation (\ref{eq_nq}). Since in ARDT:
\begin{align}
    \widetilde{Q}_{\nu^*}({s_t}, a_t) &=  \min_{\substack{\bar{a} \in \bar{\mathcal{A}}: \\ \bar{\pi}_\mathcal{D}(\bar{a} \mid s_t, a_t) > 0}} {Q}_{\omega^*}({s_{t}},a_{t}, \bar{a}), \\ 
    Q_{\omega^*}({s_t}, a_t, \bar{a}_t)  &= \max_{\substack{a' \in \mathcal{A}: \\ \pi_\mathcal{D}(a' \mid {s_{t+1}}) > 0}} \mathbb{E}_{s_{t+1} \sim \rho^{\pi_\mathcal{D}, \bar{\pi}_{\mathcal{D}}}({s_t}, a_t, \bar{a}_t)} \left[\widetilde{Q}_{\nu^*}({s_{t+1}},a') + r_t\right],
\end{align}
we have
\begin{align}
    Q_{\omega^*}({s_t}, a_t, \bar{a}_t)  = \mathbb{E}_{s_{t+1} \sim \rho^{\pi_\mathcal{D}, \bar{\pi}_{\mathcal{D}}}({s_t}, a_t, \bar{a}_t)} \left[\max_{\substack{a' \in \mathcal{A}: \\ \pi_\mathcal{D}(a' \mid {s_{t+1}}) > 0}} \min_{\substack{\bar{a} \in \bar{\mathcal{A}}: \\ \bar{\pi}_\mathcal{D}(\bar{a} \mid s_t, a_t) > 0}} {Q}_{\omega^*}({s_{t}},a_{t}, \bar{a}) + r_t\right]
\label{ardt:q_bar}
\end{align}
Comparing Eq. \eqref{ardt:q_bar} and Eq. \eqref{eq_nq}, the expectile regression in ARDT is an instance of Nash Q Learning on a in-sample game constructed by the dataset, via setting $\eta_t=1$ and deterministic policy.


